On the nature of the X(3872) from QCD

We have studied some possible four-quark and molecule contents of the X(3872) using double ratios of sum rules, which are more accurate than the usual simple ratios often used in the literature for getting the hadron masses. We found that the different structures (\bar 3-3 and \bar 6-6 tetraquarks and D-D^{(*)} molecule) lead to the same prediction for the mass (within the accuracy of the method), indicating that the alone prediction of the X mass may not be sufficient to reveal its nature. In doing these analyses, we also find that (within our approximation) the use of the \bar{MS} running {\bar m}_c(m_c^2), rather than the on-shell mass, is more appropriate to obtain the J/\psi and X meson masses. Using vertex sum rules to roughly estimate the X(3872) hadronic and radiative widths, we found that the available experimental data does not exclude a \lambda-J/\psi-like molecule current.

==> bib_x.tex <==
%%%%%%%%%%%%%%%
\begin{thebibliography}{999}
\vspace*{-0.25cm}
%%%%%%%%%%%%%%%%%%%
% EXPERIMENT
%%%%%%%%%%%%%%%%%%%
\bibitem{PDG} For a review, see e.g. PDG 08, C. Amsler et al., {\it Phys. Lett.} {\bf B 667} (2008) 1.
\bibitem{BELLE}  S.-K. Choi  {\it et al.} [Belle Collaboration],   
Phys. Rev. Lett. {\bf 91}, 262001 (2003).
\bibitem{BABAR}  B.~Aubert {\it et al.}  [{\sc {\sc BaBar}} Collaboration],
  Phys.\ Rev.\ D {\bf 71}, 071103 (2005).
\bibitem{CDF}D. Acosta {\it et al.} [CDF II Collaboration], Phys. Rev. Lett. 
{\bf 93}, 072001 (2004);
\bibitem{D0} 
 V.~M.~Abazov {\it et al.}  [D0 Collaboration],
  Phys.\ Rev.\ Lett.\  {\bf 93}, 162002 (2004);

%%%%%%%%%%%%%%%%%%%%
% REVIEW 4-QUARK
%%%%%%%%%%%%%%%%%%%
\bibitem{Swanson}
 For reviews, see e.g.,  E.~S.~Swanson,
  Phys.\ Rept.\  {\bf 429}, 243 (2006); J.~M.~Richard, talk given at QCD 05 
(Montpellier 4-8th July 2005), hep-ph/0601043.
\bibitem{rev} For a review, see e.g. M. Nielsen, F. S. Navarra, S. H. Lee, arXiv: 0911.1958.
%%%%%%%%%%%%%%%%%%%
% QSSR SVZ & REVIEW
%%%%%%%%%%%%%%%%%%%
\bibitem{svz} M.A. Shifman, A.I. and Vainshtein and V.I. Zakharov,
Nucl. Phys. {\bf B147}, 385 (1979).

\bibitem{rry} L.J. Reinders, H. Rubinstein and S. Yazaki, Phys. Rept. 
{\bf 127}, 1 (1985). 

\bibitem{SNB} For a review and references to original works, see
e.g., S. 
Narison, {\it QCD as a theory of hadrons,
Cambridge Monogr. Part. Phys. Nucl. Phys. Cosmol.} {\bf 17}, 1-778
(2002) 
[hep-h/0205006]; {\it QCD
spectral sum rules ,  World Sci. Lect. Notes Phys.} {\bf 26}, 1-527
(1989);
{ Acta Phys. Pol.} {\bf B26} (1995) 687; { Riv. Nuov. Cim.} {\bf 10N2} 
(1987) 1; { Phys. Rept.} {\bf 84}, 263 (1982).
%%%%%%%%%%%%%%%%%
%  4-QUARKS
%%%%%%%%%%%%%%%%

\bibitem{mnnr} R.D. Matheus, S. Narison, M. Nielsen, J.M. Richard,
Phys. Rev. {\bf D75}, 014005 (2007).

\bibitem{SN4} S. Narison, Phys. Lett. {\bf B175}, 88 (1986).

\bibitem{x24} R. D. Matheus, F. S. Navarra, M. Nielsen, C. M. Zanetti,
Phys. Rev. {\bf D80}, 056002 (2009).

%%%%%%%%%%%%%%
% PSI SUM RULES
%%%%%%%%%%%%%%
\bibitem{BELL}J.S. Bell and R.A. Bertlmann, {\it Nucl. Phys.} {\bf B 227}, (1983) 435; R.A. Bertlmann, {\it Acta Phys. Austriaca} {\bf 53}, (1981) 305;  R.A. Bertlmann and H. Neufeld, {\it Z. Phys.} {\bf C 27} (1985) 437.
%\bibitem{SNGh} S. Narison, {\it Phys. Lett.} {\bf B 387} (1996) 162.
\bibitem{SNGh} S. Narison, {\it Phys. Lett.} {\bf B 387} (1996) 162.
 \bibitem{FNR}E.G. Floratos, S. Narison and E. de Rafael, {\it Nucl. Phys.} {\bf B 155} (1979) 155.
 %%%%%%%%%%%%%%%%%%%
%  TACHYONIC
%%%%%%%%%%%%%%%%%%%
 \bibitem{CNZ} K. Chetyrkin, S. Narison and V.I. Zakharov, {\it Nucl. Phys.} {\bf B 550} (1999)
353;  S. Narison and V.I. Zakharov, {\it Phys. Lett.} {\bf B 522},  (2001) 266; S. Narison and V.I. Zakharov, {\it Phys. Lett.} {\bf B 679},  (2009) 355.
\bibitem{ZAK} For reviews, see e.g.: V.I. Zakharov, {\it Nucl. Phys. Proc. Suppl.} {\bf 164} (2007) 240; S. Narison,  {\it Nucl. Phys. Proc. Suppl.} {\bf 164},  225 (2007). 
% \bibitem{SNZ1} S. Narison and V.I. Zakharov, {\it Phys. Lett.} {\bf B 522},  (2001) 266.




%%%%%%%%%%%%%%%%%%
%  QCD INPUTS
%%%%%%%%%%%%%%%%%%
\bibitem{SNTAU}S. Narison, {\it Phys. Lett.} {\bf B 673} (2009) 30.
%\bibitem{HBARYON} R.M. Albuquerque, S. Narison, M. Nielsen, Phys. Lett.  {\bf B 684}, 236 (2010).

 \bibitem{SNmass} For reviews, see e.g.: S. Narison, {\it Phys.Rev.} {\bf D 74} (2006) 034013; 
 {\it arXiv:hep-ph 0202200};  {\it Phys. Lett.} {\bf B 216} (1989) 191; {\it Phys. Lett.} {\bf B 358} (1995) 113; {\it Phys. Lett.} {\bf B 466} (1999) 345; S. Narison, H.G. Dosch, {\it Phys. Lett.} {\bf B 417} (1998) 173; 
S. Narison, N. Paver, E. de Rafael and D. Treleani, {\it Nucl. Phys.} {\bf B 212} (1983) 365; S. Narison, E. de Rafael, {\it Phys. Lett.} {\bf B 103} (1981) 57; C. Becchi, S. Narison, E. de Rafael, F.J. Yndurain, {\it Z. Phys.} {\bf C 8} (1981) 335.

\bibitem{JAMI2}Y. Chung et al.{\it Z. Phys.} {\bf C 25} (1984) 151;  H.G. Dosch, Non-Perturbative Methods (Montpellier 1985);  
H.G. Dosch, M. Jamin and S. Narison, {\it Phys. Lett.} {\bf B  220} (1989) 251.
\bibitem{HEID}B.L. Ioffe, {\it Nucl. Phys.} {\bf B 188} (1981) 317 , {\bf
B 191} (1981) 591; A.A.Ovchinnikov and A.A.Pivovarov,
{\it Yad.\ Fiz.}  {\bf 48} (1988) 1135.
\bibitem{SNhl}S. Narison, Phys. Lett. {\bf B 210}, 238 (1988); Phys. Lett. {\bf B 605}, 319 (2005).
\bibitem{LNT}G. Launer, S. Narison and R. Tarrach, {\it Z. Phys.} {\bf C 26} (1984) 433.
\bibitem{SNI}S. Narison, {\it Phys. Lett.} {\bf B 300} (1993) 293; ibid {\bf B 361} (1995) 121.
\bibitem{fesr} R.A. Bertlmann, G. Launer and E. de Rafael, 
{\it Nucl. Phys.} {\bf B 250} (1985) 61; R.A. Bertlmann et al., 
{\it Z.\ Phys.}  {\bf C 39} (1988) 231.
\bibitem{YNDU}F.J. Yndurain, hep-ph/9903457.
\bibitem{SNHeavy}S. Narison, {\it Phys. Lett.} {\bf B 387} (1996) 162.
%\bibitem{BB}J.S. Bell and R.A. Bertlmann, {\it Nucl. Phys.} {\bf B 177} (1981) 218.
%{\bf B187} (1981) 285; R.A. Bertlmann, {\it Acta Phys. Austr.} {\bf 53} (1981) 305.
\bibitem{SNH10}S. Narison,  {\it arXiv:1004.5333 [hep-ph] } (2010) and references therein.
\bibitem{SNG} S. Narison, { Phys. Lett.} {\bf B361}, 121 (1995);
%S. Narison, Phys. Lett. {\bf B387}, 162 (1996). S. Narison, 
 {Phys.Lett.} {\bf B624} (2005) 223.
\bibitem{SNHmass}S. Narison, {\it Phys. Lett.} {\bf B 197} (1987) 405; {\bf Phys. Lett.} {\bf B 341} (1994) 73; {\it Phys. Lett.} {\bf B 520} (2001) 115.



%%%%%%%%%%%%%%%%%
%  PSI SUM RULE
%%%%%%%%%%%%%%%%%
%\bibitem{SNc10} S. Narison, {\it arXiv:1004.5333 [hep-ph] } (2010).
\bibitem{IOFFE} B.L. Ioffe and K.N. Zyablyuk, {\it Eur. Phys. J.} {\bf  C 27} (2003) 229; B.L. Ioffe, {\it Prog. Part. Nucl. Phys.} {\bf 56} (2006) 232.




%%%%%%%%%%%%%%%%%%%
% DOUBLE RATIOS OF SUM RULES
%%%%%%%%%%%%%%%%%%%
\bibitem{SNFBS} S. Narison, {\it Phys. Lett.} {\bf B 322} (1994) 327.
\bibitem{SNFORM} S. Narison, {\it Phys. Lett.} {\bf B 337} (1994) 166; {\it Phys. Lett.} {\bf B 668} (2008) 308.
\bibitem{SNme+e-} S. Narison, {\it Phys.Rev.} {\bf D 74} (2006) 034013; {\it Phys. Lett.} {\bf B 358} (1995) 113; {\it Phys. Lett.} {\bf B 466} (1999) 34.
\bibitem{HBARYON}R.M. Albuquerque, S. Narison, M. Nielsen, {\it Phys. Lett.} {\bf B 684} (2010) 236.


%%%%%%%%%%%%%%%%%%%
% DOUBLE RATIOS OF SUM RULES
%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%
% VERTEX SUM RULES
%%%%%%%%%%%%%%%%%%
\bibitem{NN}F. Navarra and M. Nielsen, {\it Phys. Lett.} {\bf B 639} (2006) 272.

\end{thebibliography}
\end{document}
















%%%%%%%%%%%%%%%%%%%
% QCD PARAMETERS CONTINUED
%%%%%%%%%%%%%%%%%%%
%\bibitem{SNhl}S. Narison, Phys. Lett. {\bf B 210}, 238 (1988); Phys. Lett.  {\bf B 605}, 319 (2005).
\bibitem{SNCB} S. Narison,  { Nucl. Phys. Proc. Suppl.} {\bf 86}, 242 (2000); 
S. Narison, hep-ph/0202200; S. Narison, hep-ph/0510108; 
S. Narison, {Phys. lett.} {\bf B341}, 73  (1994); H.G. Dosch and S. Narison,
{Phys. lett.} {\bf B417}, 173  (1998); S. Narison,	{Phys. lett.} 
{\bf B216}, 191  (1989); S. Narison, Phys. Lett. {\bf B466}, 345 (1999).








%%%%%%%%%%%%%%%%
%  QCD PARAMETERS
%%%%%%%%%%%%%%%
%\bibitem{LNT} G. Launer, S. Narison and R. Tarrach, Z. Phys. {\bf C 26}, 433
 (1984).

\bibitem{SNTAU} S. Narison, Phys. Lett. {\bf B 673}, 30 (2009).
\bibitem{DOSCH} Y. Chung et al., {\it Phys. Lett.} {\bf B 102} (1981) 175; {\it Nucl. Phys.} {\bf B 197} (1982) 55; H.G. Dosch, Non-Perturbative Methods (Montpellier 1985);  H.G. Dosch, M. Jamin and S. Narison, {\it  Phys. Lett.} {\bf B 220} (1989) 251.




\bibitem{SVZ}M.A. Shifman, A.I. Vainshtein and V.I. Zakharov, {\it Nucl. Phys.} {\bf B 147} (1979) 385, 448.
\bibitem{ZAKA}For a review, see e.g.: V.I. Zakharov, talk given at the Sakurai's Price, {\it Int. J. Mod .Phys.} {\bf  A 14}, (1999) 4865.

\bibitem{SNB1}For a review, see e.g.: S. Narison, {\it Cambridge Monogr. Part. Phys. Nucl. Phys. Cosmol.} {\bf 17}
 (2004) 1-778 [hep-ph/0205006]. 
 \bibitem{SNB2}For a review, see e.g.: S. Narison, {\it World Sci. Lect. Notes Phys.} {\bf 26} (1989) 1.
\bibitem{SNB3}For a review, see e.g.: S. Narison, {\it Acta Phys. Pol.} {\bf B 26}(1995) 687;  S. Narison, {\it Phys. Rept.}  {\bf 84} (1982) 263. 

%%%%%%%%%%%%%%%%%%%
% GLUON CONDENSATE
%%%%%%%%%%%%%%%%%%%
\bibitem{BELL}J.S. Bell and R.A. Bertlmann, {\it Nucl. Phys.} {\bf B 227}, (1983) 435; R.A. Bertlmann, {\it Acta Phys. Austriaca} {\bf 53}, (1981) 305.
\bibitem{SNHeavy} S. Narison, {\it Phys. Lett.} {\bf B 387} (1996) 162.
%%%%%%%%%%%%%%%%%%%%%%%%%%
\bibitem{LNT}G. Launer, S. Narison and R. Tarrach, {\it Z. Phys.} {\bf C 26} (1984) 433.
%M. Kremer, N.A. Papadopoulos and K. Schilcher, {\it  Phys. Lett.} {\bf B 143}, 476 (1984); 
\bibitem{PEROTTET}R.A. Bertlmann, G. Launer and E. de Rafael, {\it Nucl. Phys.} {\bf B 250}, (1985) 61 ;
R.A. Bertlmann et al., {\it Z. Phys.} {\bf C 39}, (1988) 231.
\bibitem{SNI}S. Narison, {\it Phys. Lett.} {\bf B 300} (1993) 293; {\it Phys. Lett.}  {\bf B 361} (1995) 121.
% and references therein.
\bibitem{ALEPH} The ALEPH collaboration, S. Schael et al., {\it Phys. Rept.} {\bf 421}, 191 (2005).
\bibitem{OPAL} The OPAL collaboration, K. Ackerstaff et al., {\it Eur. Phys. J} {\bf C 8}, 183 (1999).
\bibitem{DAVIER}M. Davier et al., {\it Eur. Phys. J.} {\bf C 56},  (2008) 305.
\bibitem{SNTAU}S. Narison, {\it Phys. Lett.} {\bf B 673} (2009) 30.
\bibitem{IOFFE} B.L. Ioffe and K.N. Zyablyuk, {\it Eur. Phys. J.} {\bf  C 27} (2003) 229; B.L. Ioffe, {\it Prog. Part. Nucl. Phys.} {\bf 56} (2006) 232.
 \bibitem{CNZ} K. Chetyrkin, S. Narison and V.I. Zakharov, {\it Nucl. Phys.} {\bf B 550} (1999)
353;  S. Narison and V.I. Zakharov, {\it Phys. Lett.} {\bf B 522},  (2001) 266; S. Narison and V.I. Zakharov, {\it Phys. Lett.} {\bf B 679},  (2009) 355.
\bibitem{SNREV} For reviews, see e.g.: V.I. Zakharov, {\it Nucl. Phys. Proc. Suppl.} {\bf 164} (2007) 240; S. Narison,  {\it Nucl. Phys. Proc. Suppl.} {\bf 164},  225 (2007). 
 \bibitem{SNZ1} S. Narison and V.I. Zakharov, {\it Phys. Lett.} {\bf B 522},  (2001) 266.
 \bibitem{RAF04}S. Friot, D. Greynat and E. de Rafael, {\it JHEP} {\bf 10},  (2004) 043; 
 M. Gonzalez-Alonso, A. Pich and J. Prades, {\it arXiv:} 1004.4987 [hep-ph] (2010).
\bibitem{SNVA}S. Narison, {\it Phys. Lett.} {\bf B 624},  (2005) 223.
\bibitem{BORDES}J. Bordes, V. Gimenez, J.A. Penarrocha, {\it Phys. Lett.} {\bf B 201} (1988) 365.
\bibitem{MENES} M.B. Causse and G. Mennessier, {\it Z. Phys.} {\bf C 47} (1990) 611.
\bibitem{DOMI}C.A. Dominguez and J. Sol\'a, {\it Z. Phys.} {\bf C 40} (1988) 63.
\bibitem{DOSCH} Y. Chung et al., {\it Phys. Lett.} {\bf B 102} (1981) 175; {\it Nucl. Phys.} {\bf B 197} (1982) 55; H.G. Dosch, Non-Perturbative Methods (Montpellier 1985);  H.G. Dosch, M. Jamin and S. Narison, {\it  Phys. Lett.} {\bf B 220} (1989) 251.
\bibitem{GIACO} A. Di Giacomo, Non-pertubative Methods, ed. Narison, World Scientific (1985); M. Campostrini, A. Di Giacomo, Y. Gunduc {\it Phys. Lett.} {\bf B 225} (1989) 393; A. Di Giacomo and G.C. Rossi, {\it Phys. Lett.} {\bf B 100} (1981) 481.
\bibitem{GIACO3}Private communication from  A. Di Giacomo.
\bibitem{GIACO2}M. D'Elia, A. Di Giacomo and E. Meggiolaro, {\it Phys. Lett.} {\bf B 408} (1997) 315. 
%and private communication from Adriano Di Giacomo.
\bibitem{RAKOW} P.E. Rakow, {\it arXiv:hep-lat/0510046 }; G. Burgio, F. Di Renzo, G. Marchesini and E. Onofri, {\it Phys. Lett.} {\bf B 422} (1998) 219; R. Horley, P.E.L. Rakow and G. Schierholz, {\it Nucl. Phys. (Proc. Sup.)} {\bf B 106} (2002) 870.
\bibitem{SHURYAK}T. Schafer and E.V. Shuryak, {\it Rev. Mod. Phys.} {\bf 70} (1998) 323.
\bibitem{IOFFE2}B.L. Ioffe and A.V. Samsonov, {\it Phys. At. Nucl.} {\bf 63} (2000) 1448.
\bibitem{PDG} PDG, C. Amsler et al., {\it Phys. Lett.} {\bf B 667} (2008) 1.
\bibitem{KUHN}K. Chetyrkin, J.H. Kuhn and M. Steinhauser, {\it Nucl. Phys.} {\bf B 505} (1997) 40. 
\bibitem{KUHN1}K.G. Chetyrkin et al., {\it Phys. Rev} {\bf D 80} (2009) 074010; J.H. Kuhn, M. Steinhauser and C. Sturm, {\it Nucl. Phys.} {\bf B 778} (2007) 192;
A. Maier, P. Mairhofer and P.Marquard, {\it Phys. Lett.} {\bf B 669} (2008) 88; 
A. Signer, {\it Phys. Lett.} {\bf B 672} (2009) 333.
\bibitem{KUHN2}K. Chetyrkin, J.H. Kuhn and C. Sturm, {\it Eur. Phys.} {\bf C 48} (2006) 107.
\bibitem{BOUG}R. Boughezal, M. Czakon and T. Schutzmeier, {\it Phys. Rev} {\bf D 74} (2006) 074006.
\bibitem{PIVO}S. Groote and A. Pivovarov, {\it JETP Lett.} {\bf 75} (2002) 221.
\bibitem{SIGNER}A. Signer, {\it Phys. Lett.} {\bf B 654} (2007) 206.
\bibitem{RRY}L.J. Reinders, H. Rubinstein and S. Yazaki, {\it Phys. Rept. } {\bf 127} (1985) 1.
\bibitem{SNmc}S. Narison, {\it Phys. Lett.} {\bf B 197}  (1987) 405; {\it Phys. Lett.} {\bf B 216}  (1989) 191;
{\it Phys. Lett.} {\bf B 341}  (1994) 73.
\bibitem{JAMIN}M. Jamin and A. Pich, {\it Nucl. Phys.} {\bf   507} (1997) 334; 
M. Jamin and A. Hoang, {\it Phys. Lett.} {\bf B 594}  (2004) 127.
%\bibitem{BRAMBILLA} Quarkonium working group, N. Brambilla et al., hep-ph/0412158.
\bibitem{BETHKE} S. Bethke, {\it Prog. Part. Nucl. Phys.} {\bf 58} (2007) 351.
\bibitem{EICHTEN}E. Eichten et al.,{\it Phys. Rev} {\bf D 21} (1980) 203.
\bibitem{BES}The BES collaboration, J.Z. Dai et al.,  {\it Phys. Rev. Lett.} {\bf 88} (2002) 101802.
\bibitem{LATTmc}I. Allison et al., {\it Phys. Rev. } {\bf D 78} (2008) 054513.
\bibitem{SNpseudo}S. Narison, {\it Phys. Lett.} {\bf B 520}  (2001) 115.
%\bibitem{HOANG}G. Corcella and A.H. Hoang, {\it Phys. Lett.} {\bf B 554}  (2003) 133.
\bibitem{STEIN}K. Chetyrkin, J.H. Kuhn and M. Steinhauser, {\it Comput. Phys. Commun.} {\bf 133} (2000) 43.
\bibitem{SNmq}S. Narison, {\it Phys.Rev.} {\bf D 74} (2006) 034013; {\it Phys. Lett.} {\bf B 626} (2005) 101;  {\it Phys. Lett.} {\bf B 466} (1999) 345; {\it  Phys. Lett.} {\bf B 358} (1995) 113.
\bibitem{SNmq2} For earlier reviews, see e.g. S. Narison, {\it arXiv:hep-ph 0202200}; {\it Nucl. Phys. Proc. Suppl.} {\bf 86} (2000) 242; {\it Riv. Nuovo Cim.} {\bf 10N2} (1987) 1.
\bibitem{FRITZSCH}H. Fritzsch, {\it Phys. Lett.} {\bf B 73} (1978) 317; {\it Int. J. Mod. Phys.} {\bf A 25} (2010) 597.
\bibitem{CECILIA}C. Jarlskog, {\it Z. Phys.} {\bf C 29} (1985) 491; {\it Phys.Rev.} {\bf D 35} (1987) 1685;
P. Frampton and C. Jarlskog,  {\it Phys. Lett.} {\bf B 154} (1985) 421.
\bibitem{GEORGI}See e.g., H. Georgi and D.V. Nanopoulos, {\it Nucl. Phys. } {\bf B 155} (1979) 52.
\bibitem{BABAR} The BABAR collaboration, B. Aubert et al. {\it Phys. Rev. Lett.} {\bf 102} (2009) 012001.
\end{thebibliography}
\end{document}




